Frankenstein: Advanced Wireless Fuzzing to Exploit New Bluetooth Escalation Targets

Wireless communication standards and implementations have a troubled history regarding security. Since most implementations and firmwares are closed-source, fuzzing remains one of the main methods to uncover Remote Code Execution (RCE) vulnerabilities in deployed systems. Generic over-the-air fuzzing suffers from several shortcomings, such as constrained speed, limited repeatability, and restricted ability to debug. In this paper, we present Frankenstein, a fuzzing framework based on advanced firmware emulation, which addresses these shortcomings. Frankenstein brings firmware dumps "back to life", and provides fuzzed input to the chip's virtual modem. The speed-up of our new fuzzing method is sufficient to maintain interoperability with the attached operating system, hence triggering realistic full-stack behavior. We demonstrate the potential of Frankenstein by finding three zero-click vulnerabilities in the Broadcom and Cypress Bluetooth stack, which is used in most Apple devices, many Samsung smartphones, the Raspberry Pis, and many others. Given RCE on a Bluetooth chip, attackers may escalate their privileges beyond the chip's boundary. We uncover a Wi-Fi/Bluetooth coexistence issue that crashes multiple operating system kernels and a design flaw in the Bluetooth 5.2 specification that allows link key extraction from the host. Turning off Bluetooth will not fully disable the chip, making it hard to defend against RCE attacks. Moreover, when testing our chip-based vulnerabilities on those devices, we find BlueFrag, a chip-independent Android RCE.

==> sections/demo.tex <==
%!TEX root = ../fuzzing_coex.tex

\clearpage
\newpage

\section{Appendix: \fuzztool Demo}

%\todo{@jan: when producing new screenshots, high resolution is one thing, but also try a smaller terminal width... or maybe we just copy outputs and use listings? i also think that white background would work better in a paper.}

In this appendix, we give a brief overview on \fuzztool's capabilities.
Upon acceptance of this paper, we will publish the source code along with
detailed examples for \cvea and \cveb.
Nonetheless, we already want to provide some insights to the curious reader.

\subsection{Memory Layout Setup}

A basic web front-end assists in setting up the memory layout.
Memory segments can be imported either from raw dumps or \ac{ELF} files including symbols.
The setup is saved in a machine readable \ac{JSON} file format and the linker scripts are generated automatically.

\begin{figure}[h!]
\center
\includegraphics[width=1.0\columnwidth]{demo/webfrontend.png}
\caption{\fuzztool frontend for memory layout setup.}
\end{figure}

While the \emph{CYW20735} Bluetooth firmware is emulated, \fuzztool will generate various outputs.
These are annotated with symbols extracted from \emph{WICED Studio}.
Moreover, execution stops with debug printouts and a memory dump once a heap overflow is detected.


\subsection{State Snapshot}

The \path{xmit_state} hook used for generating snapshots is shown in \autoref{lst:xmit_state}.
This function saves all registers to the stack and provides a return point to the firmware state. To take control over registers, it needs to be written in inline Assembly.

\begin{figure}[!b]
\begin{lstlisting}[caption=Assembly patch for creating a re-executable state on a physical Bluetooth controller., label=lst:xmit_state, language=ASM]
@\textbf{xmit\_state}@:
push {r0-r12,lr}
ldr r0, =saved_regs
str sp, [r0]

// Send memory to host using HCI and disable interrupts
bl @\textbf{xmit\_memory}@

// This is our re-entrance point
@\textbf{cont}@:
ldr r0, =saved_regs
ldr sp, [r0]
pop {r0-r12,pc}
\end{lstlisting}
\end{figure}




\subsection{\acl{BCS} Abstraction}

Valid input according to the calling convention is generated by running the code shown in \autoref{lst:bcs} in an endless loop.
The function \path{read_linux} reads data the \emph{Linux} host passes over a given file descriptor.
Based on this \ac{BCS} abstraction, we are able to fuzz arbitrary payloads as if they arrived over the air.
Furthermore, we are able to analyze the time-critical \ac{ACL} state machine in the emulation.

\begin{figure}[!b]
\begin{lstlisting}[caption={Bluetooth Core Scheduler (BCS) packet injection, running as endless loop.}, label={lst:bcs}]
pcx_btclk++;                            // advance BT clock
@\vspace{-0.5em}@
if (pcx_btclk & 0b11 == 0b00) {
  phy_status = @\textcolor{red!70!black}{RX\_HDR\_DONE}@;
  read_linux(0, &pkt_log, 2);           // packet header
  read_linux(0, &pkt_hdr_status, 2);    // payload header
}
@\vspace{-0.5em}@
if (pcx_btclk & 0b11 == 0b01) {
  phy_status = @\textcolor{red!70!black}{RX\_DONE}@;
  read_linux(0, dmaActiveRxBuffer, 240); // packet data
}
@\vspace{-0.5em}@
if (pcx_btclk & 0b11 == 0b10)phy_status = @\textcolor{red!70!black}{TX\_DONE}@;
if (pcx_btclk & 0b11 == 0b01)phy_status |= @\textcolor{red!70!black}{SLOT\_01\_INT}@;
if (pcx_btclk & 0b11 == 0b11)phy_status |= @\textcolor{red!70!black}{SLOT\_11\_INT}@;
@\vspace{-0.5em}@
@\textbf{bluetoothCoreInt\_C()}@;                    // invoke interrupt
\end{lstlisting}
\end{figure}

\subsection{Device Scanning Operation}

To start \fuzztool and feed it random wireless input, it can be started as follows:
\begin{lstlisting}
cat /dev/random | qemu-arm hci_attach.exe
\end{lstlisting}

This will start the emulator, redirect \ac{HCI} messages to a \ac{PTS} and run \texttt{btattach} on the resulting master device.
A new \ac{HCI} device will be created, which can be used with the \emph{BlueZ} stack on \emph{Linux} to some extent.
Now, we can use the emulated firmware as \ac{HCI} device and perform further actions, i.e., device scanning.
With the random wireless input provided, this will generate valid outputs during a device scan, as shown in \autoref{lst:lescan}.
Running this setup produces a lot of \texttt{lescan} results within short time.
A very verbose \fuzztool emulation output with annotated firmware insights is generated as shown in \autoref{lst:hci_lm_states}.
It is possible to follow basic block execution. Moreover, events of interest are highlighted, such as context switches or data transferred from and to the host.




\begin{figure}[!b]
% space in HCI event is to create line break
% !!!!!!! The console output matches the console dump above (last scan result)
\begin{lstlisting}[linewidth=\columnwidth, language=none, label=lst:lescan, caption={Performing an \texttt{lescan}. Random advertisement reports generated by \fuzztool are ``received''. }]
# hciconfig hci1 up
Can't get device info: No such device
@\textcolor{gray}{< Starting emulator in other shell >}@
# hciconfig hci1 up
# hcitool -i hci1 lescan
LE Scan ...
4E:4B:59:8E:E5:FF (unknown)
29:19:1D:83:E6:E7 (unknown)
10:17:1F:46:D8:71 (unknown)
DA:2C:F4:69:4D:07 (unknown)
\end{lstlisting}
\end{figure}




\subsection{Analyzing Vulnerabilities}
We can put the \ac{BLE} emulation one step further and try to establish connections to the devices generated and reported by \fuzztool during scanning.
During fuzzing, the \ac{BCS} kernel will eventually create a valid connection after a couple of attempts.
On the \emph{Linux} host, we try to establish a connection in an endless loop.

\begin{lstlisting}[linewidth=0.97\columnwidth, language=none]
while [ 1 -eq 1 ]; do hcitool -i hci1 lecc 00:11:22:33:44:55; done
\end{lstlisting}


Using this technique, we were able to detect \emph{CVE-2019-xxx2} within a few minutes on a \emph{Thinkpad T430} with an \emph{i5-3320M} CPU. \autoref{lst:blepdufuzz} shows the output leading to the according \ac{BLE} \ac{PDU} heap corruption.
\fuzztool stops execution upon heap corruption and we can further analyze the issue.

Note that in this setup, the challenge is no longer to locate the heap corruption, since \fuzztool does that with high performance. However, successfully setting up a connection based on \ac{BLE} device scan fuzzing inputs takes a while. Once a connection is set up, it only takes around \SI{7}{\second} to detect the vulnerability.

%Hard step here is to setup an LE connection. As the connection is set up it either takes ~7secs to detect the Heap BoF or the firmware hangs for some reason.


%\todo{why does establishing a connection to 00:11:22:33:44:55 with random data actually work? do establishments need to be answered correctly or are invalid answers already parsed somehow?
%Answer: I haven't fully understood the connection setup yet. But I noticed by 'fuzzing' the paging tasks, I sometimes create a new connection and then I found the LE bug, so i shifted my focus on that... This can be definetly improved at some point.
%}


\begin{figure*}[!b]
\begin{lstlisting}[linewidth=\textwidth,alsoletter={()[].=},label=lst:hci_lm_states,caption={\fuzztool emulator answering the \texttt{lescan}. The emulator output shows how the packet is handed from the \ac{BCS} kernel to the \ac{HCI}.}]
tb = bcsulp_scan
Rx Done
wib_rx_status = 0xe9a42580
wib_pkt_log = 0xeb3f9acf
@\textcolor{blue!80}{{lr=0x040165 bcs\_kernelRxDone()lr=0x096e2d \_scanTaskRxDone(0x283300, 0x075a2b, 0x01)lr=0x0549f5 utils\_memcpy8(0x24dca0, 0x370c00, 0x0100);}}@
@\textcolor{blue!80}{{lr=0x054a2b bcsulp\_getPktLength(0x2580, 0x01) = 0x25;}}@
@\textcolor{blue!80}{{lr=0x054a37 dynamic\_memory\_AllocateOrDie(0x2f) = 0x21fb50;}}@
@\textcolor{blue!80}{{lr=0x054a51 \_\_rt\_memcpy(0x21fb50, 0x24dca0, 0x2b);}}@
lr = 0x054a7b lm_sendCmd(0x0d | 0x2580 | 0x0400);
@\textcolor{blue!80}{{lr=0x048d11 dynamic\_memory\_AllocateOrDie(0x18) = 0x21fb1c;}}@
@\textcolor{red!70!black}{{Context switch idle -$>$ lm}}@
@\textcolor{blue!80}{{lr=0x02cccf dynamic\_memory\_Release(0x21fb1c);}}@
@\textcolor{blue!80}{{lr=0x055b8b \_\_rt\_memcpy(0x20c54a, 0x21fb56, 0x1f);}}@
@\textcolor{blue!80}{{lr=0x02df01 dynamic\_memory\_AllocateOrDie(0x2d) = 0x21fb1c;}}@
@\textcolor{blue!80}{{lr=0x0ca7f9 \_\_rt\_memcpy(0x21fb29, 0x20c54a, 0x1f);}}@
@\textcolor{blue!80}{{lr=0x02decd dynamic\_memory\_AllocateOrReturnNULL(0x35) = 0x220204;}}@
@\textcolor{blue!80}{{lr=0x02dee5 \_\_rt\_memcpy(0x22020c, 0x21fb1c, 0x2d);}}@
@\textcolor{blue!80}{{lr=0x02deeb bthci\_event\_AttemptToEnqueueEventToTransport(0x220204)}}@
@\textcolor{blue!80}{{lr=0x024ce9 mpaf\_hci\_EventFilter(0x24fbe8, 0x0265af, 0x3d, 0x1d) = 0x0;}}@
@\textcolor{blue!80}{{lr=0x024df7 bttransport\_SendMsgToThread(0x220204, 0x0)}}\textcolor{red!70!black}{{Context switch lm -$>$ bttransport}}@
@\textcolor{blue!80}{{lr=0x01960d btuarth4\_RunTxStateMachines(0x249e58, 0x01, 0x0, 0x0)lr=0x019265 uart\_SendAsynch(0x249f70, 0x249e10, 0x01, 0x22020c)}}\textcolor{green!80!black}{HCI Event (Asynch)043e2b02010000074d69f42cda1ffc563137b934e0f5302dfbf4498210cb6163843cbbf1fec7590d1bd957930b00}@
@\textcolor{blue!80}{{lr=0x03fd03 uart\_SendSynchHeaderBeforeAsynch(0x249f70, 0x249e10, 0x01, 0x2d);}}@
@\textcolor{blue!80}{{lr=0x062c1d uart\_DirectWrite(0x22020c, 0x2d) = 0x22020c;}}@
@\textcolor{blue!80}{{= 0x0;}}@
@\textcolor{blue!80}{{lr=0x0193fb dynamic\_memory\_Release(0x220204);}}@
@\textcolor{blue!80}{{= 0x80000000;}}@
@\textcolor{blue!80}{{lr=0x01de2d btuarth4\_RunRxStateMachines(0x249e58) = 0x88000000;}}@
@\textcolor{red!70!black}{{Context switch bttransport -$>$ lm}}@
@\textcolor{blue!80}{{;}}@
@\textcolor{blue!80}{{;}}@
@\textcolor{blue!80}{{lr=0x0ca819 dynamic\_memory\_Release(0x21fb1c);}}@
@\textcolor{blue!80}{{lr=0x02ccd9 dynamic\_memory\_Release(0x21fb50);}}@
@\textcolor{red!70!black}{{Context switch lm -$>$ idle}}@
\end{lstlisting}
\end{figure*}


\begin{figure*}[h]
\begin{lstlisting}[linewidth=1.0\textwidth,label=lst:blepdufuzz,caption={Heap corruption when receiving a \ac{BLE} \ac{PDU}, leading to \emph{CVE-2019-xxx2}.}]
@\textcolor{blue!80}{{lr=0x08e2d3 bcsulp\_setupRxBuffer()lr=0x08dfaf dhmulp\_getRxBuffer(0x0)lr=0x0bf018f5 mmulp\_allocACLUp(0x0108)lr=0x016ea5 dynamic\_memory\_SpecialBlockPoolAllocateOrReturnNULL (0x20d38c) = 0x2232c4;}}@
@\textcolor{blue!80}{{= 0x2232cc;}}@
@\textcolor{blue!80}{{= 0x2232cc;}}@
@\textcolor{blue!80}{{= 0x03;}}@
@\textcolor{blue!80}{{= 0x02000000;}}@
@\textcolor{gray}{[...]}@
Rx Done
wib_rx_status = 0x85f9ffcf
wib_pkt_log = 0x751eb6be
@\textcolor{blue!80}{{lr=0x040165 bcs\_kernelRxDone()lr=0x08ee3d bcsulp\_getPktLength(0x85f9ffcf, 0x0) = 0xff;}}@
@\textcolor{blue!80}{{lr=0x08ed33 bcsulp\_getPktLength(0x0d, 0x0) = 0x0;}}@
@\textcolor{blue!80}{{lr=0x041e95 bcsulp\_getPktLength(0x85f9ffcf, 0x0) = 0xff;}}@
@\textcolor{blue!80}{{lr=0x08f115 bcsulp\_procRxPayload(0x281618, 0x85f9ffcf)lr=0x08e9c3 bcsulp\_getPktLength(0x85f9ffcf, 0x0) = 0xff;}}@
@\textcolor{blue!80}{{lr=0x08ea2f bcsulp\_getPktLength(0x85f9ffcf, 0x0) = 0xff;}}@
@\textcolor{blue!80}{{lr=0x08ea4b utils\_memcpy8(0x2232d0, 0x370c00, 0xff)}}@@\textcolor{red!70!black}{Heap Corruption Detected}@
pool = 0x20d38c
pool->block_start = 0x2232c0
pool->capacity = 0x0f
pool->size = 0x0108
free_chunk = 0xa09b9af8

@\textcolor{red!70!black}{\textbf{qemu: uncaught target signal 11 (Segmentation fault) - core dumped}}@
\end{lstlisting}
\end{figure*}



